Coordinating Filters for Faster Deep Neural Networks

Very large-scale Deep Neural Networks (DNNs) have achieved remarkable successes in a large variety of computer vision tasks. However, the high computation intensity of DNNs makes it challenging to deploy these models on resource-limited systems. Some studies used low-rank approaches that approximate the filters by low-rank basis to accelerate the testing. Those works directly decomposed the pre-trained DNNs by Low-Rank Approximations (LRA). How to train DNNs toward lower-rank space for more efficient DNNs, however, remains as an open area. To solve the issue, in this work, we propose Force Regularization, which uses attractive forces to enforce filters so as to coordinate more weight information into lower-rank space. We mathematically and empirically verify that after applying our technique, standard LRA methods can reconstruct filters using much lower basis and thus result in faster DNNs. The effectiveness of our approach is comprehensively evaluated in ResNets, AlexNet, and GoogLeNet. In AlexNet, for example, Force Regularization gains 2x speedup on modern GPU without accuracy loss and 4.05x speedup on CPU by paying small accuracy degradation. Moreover, Force Regularization better initializes the low-rank DNNs such that the fine-tuning can converge faster toward higher accuracy. The obtained lower-rank DNNs can be further sparsified, proving that Force Regularization can be integrated with state-of-the-art sparsity-based acceleration methods. Source code is available in https://github.com/wenwei202/caffe

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
Our similarity regularization can achieve significantly lower-rank basis in low-rank approximation to retain the same approximation error. 
However, it is also more difficult for the lower-rank DNNs to restore the accuracy. 
It is worthy to explore new algorithms to recover the accuracy of lower-rank DNNs the weight approximation of which has the same error.

Moreover, our experiments show that $\ell_2$-norm force is superior to $\ell_1$-norm force in some layers, but inferior to others. Mixing $\ell_2$-norm force and $\ell_1$-norm force in different layers may give us a better speedup.


Finally, cross validation of hyper-parameters (of both LRA and similarity regularization) is time-consuming. 
We may reduce cross validation time of LRA by integrating LRA into the training process of DNNs. 
For example, by gently removing one ignorable rank during the training, we may maintain the classification accuracy meanwhile reducing ranks to the optimal values. 
To reduce cross validation of the coefficient of regularization, we may adapt the updating step along the direction of regularization gradient to the one of classification error gradient. 
With a larger step along the direction of regularization gradient, we can obtain lower-rank DNNs and a higher error, \textit{vice versa}. 

==> method_extension.tex <==
\subsection{Generalizations of Force Regularization}
\label{method:extension}

%Adaptive hyper-parameters:
%Advantages of adaptive regularization: (1) different layers have different extent of low rank, it can adapt different strengths of regularization to different layers instead of a fixed equal value; (2) cross-validation is not required, which can reduce the training time to explore the trade-off.
In convolutional layers, each filter basically extracts a discriminative feature, \textit{e.g.}, an orientation-selective pattern or a color blob in the first layer~\cite{Alex_NIPS2012_4824} or a high-level feature (\textit{e.g.}, textures, faces, \textit{etc.}) in deeper layers~\cite{zeiler2014visualizing}. 
The discrimination among filters is important for classification performance. Our method can be generalized to learn more discriminative filters to improve the accuracy of state-of-the-art DNNs.
The extension to \textit{Discrimination Regularization} is straightforward but effective: the opposite gradient of force regularization (\textit{i.e.}, $\lambda_s<0$) is utilized to update the filter. In this scenario, it works as the \textit{repulsive force} to repel surrounding filters and enhance the discrimination.
Experimental results will be given in Section~\ref{method:accuracy}.

%Previous works show that there exist significant redundancies between filters and between channels~\cite{Max_J_arxiv2014}. Our method can be generalized to improve the similarity between channels for lower-rank approximation. 
%The generalization is simple: In Fig.~\ref{fig:similarity_reg}, instead of reshaping the $n$-th filter $\mathcal{W}_n \in \mathbb{R}^{1 \times C \times H \times W} $ as the vector $\mathbf{W}_{n} \in \mathbb{R}^{1 \times CHW}$, we can reshape weights across the $c$-th channel $\tilde{\mathcal{W}}_c \in \mathbb{R}^{N \times 1 \times H \times W}$ as a vector $\mathbf{W}_{c} \in \mathbb{R}^{1 \times NHW}$, and then follow the same optimization.


==> regularization.tex <==
\section{Fore Regularization on Filters}
\label{sec:method}

% 3-3.5 pages

% Proposed force regularization

% Math proof about the gradient direction & matrix formulation 

% Extension: degrdation + constant

\subsection{Adaptive Force Regularization}
Advantages of adaptive regularization: (1) different layers have different extent of low rank, it can adapt different strengths of regularization to different layers instead of a fixed equal value; (2) cross-validation is not required, which can reduce the training time to explore the trade-off.

